Pattern Unification for the Lambda Calculus with Linear and Affine Types

We define the pattern fragment for higher-order unification problems in linear and affine type theory and give a deterministic unification algorithm that computes most general unifiers.

==> eptcsdata.tex <==
\providecommand{\firstpage}{101}
\providecommand{\publicationstatus}{K. Crary, M. Miculan (Eds.): Logical Frameworks and\\ Meta-languages: Theory and Practice (LFMTP) 2010\\
EPTCS 34, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.34.9}{10.4204/EPTCS.34.9}}

